Collective secondary instabilities: an application to three-dimensional boundary-layer flow

In some linearly unstable flows, secondary instability is found to have a much larger wavelength than that of the primary unstable modes, so that it cannot be recovered with a classical Floquet analysis. In this work, we apply a new formulation for capturing secondary instabilities coupling multiple length scales of the primary mode. This formulation, based on two-dimensional stability analysis coupled with a Bloch waves formalism originally described in Schmid et al. (2017), allows to consider high-dimensional systems resulting from several repetitions of a periodic unit, by solving an eigenproblem of much smaller size. Collective instabilities coupling multiple periodic units can be thus retrieved. The method is applied on the secondary stability of a swept boundary-layer flow subject to stationary cross-flow vortices, and compared with Floquet analysis. Two multi-modal instabilities are recovered: for streamwise wavenumber $\alpha_v$ close to zero, approximately twelve sub-units are involved in large-wavelength oscillations; whereas a staggered pattern, characteristic of subharmonic instabilities, is observed for $\alpha_v = 0.087$.

==> main2 <==
% This is jfm2esam.bib v1.0 08/14/02
%
@Book{Schmid,
  author = 	 "Schmid, P. \& Henningson, D.",
  title = 	 "Stability and Transition in Shear Flows",
  year = 	 "2001",
  publisher = "Springer"
}

@article{Uhlmann,
    author = "Uhlmann, M. \& Nagata, M.",
    title = "Linear stability of flow in an internally heated
rectangular duct",
    journal =      "J. Fluid Mech.",
    volume =       "551",
    pages =        "387-404",
    year =         "2006"
}

@article{Monokrousos,
    author = "Monokrousos, M. \textit{et. al}",
    title = "Nonequilibrium Thermodynamics and the Optimal Path to Turbulence in Shear Flows",
    journal =      "Phys. Rev. Lett.",
    volume =       "106",
    pages =        "134502",
    year =         "2010"
}

@article{Sameen,
    author = "Sameen, A. \& Govindarajan, R.",
    title = "The effect of wall heating on instability of channel flow",
    journal =      "J. Fluid. Mech.",
    volume =       "577",
    pages =        "417-442",
    year =         "2007"
}

@article{Biau,
    author = "Biau, D. \& Bottaro, A.",
    title = "The effect of stable thermal stratification on shear flow stability",
    journal =      "Phys. Fluids.",
    volume =       "16",
    number =       "12",
    year =         "2004"
}

@book{Trefethen,
    author = "Trefethen",
    title = "Spectral methods in MATLAB",
    year =         "2001",
    publisher = "SIAM"
}

@phdthesis{Jerome,
    author = "Jerome, J.J.S.",
    title = "Transient Growth in Rayleigh-Bénard-Poiseuille/Couette flows",
    school =       "Ecole Polytechnique",
    year =         "2011"
}

@article{Onsager,
    author = "Onsager, L.",
    title = "Reciprocal relations in irreversible processes. I",
    journal =      "Phys. Rev.",
    volume =       "37",
    number =       "405",
    year =         "1931"
}

@Book{Prigogine,
  author = 	 "Prigogine, I. \& Kondepudi D.",
  title = 	 "Modern Thermodynamics: From Heat Engines to Dissipative Structures",
  year = 	 "1998",
  publisher = "Wiley"
}

@article{Goody,
    author = "Goody, R.",
    title = "Maximum Entropy Production in Climate Theory",
    journal =      "J. Atmos. Sci.",
    volume =       "64",
    pages =        "2735–2739",
    year =         "2007"
}

@article{Schmid_b,
    author = "Schmid, P. \& Brandt, L.",
    title = "Analysis of fluid systems: stability, receptivity, sensitivity",
    journal =      "Appl. Mech. Rev.",
    volume =       "66",
    number =        "024803 ",
    year =         "2014"
}

@article{Nagata,
    author = "Nagata, M. \& Generalis, S.",
    title = "Transition in Convective Flows Heated Internally",
    journal =      "J. Heat Trans.",
    volume =       "124",
    number =        "635",
    year =         "2002"
}

@article{Generalis,
    author = "Generalis, S. \& Nagata, M.",
    title = "Transition in Homogeneously Heated Inclined Plane Parallel Shear Flows",
    journal =      "J. Heat Trans.",
    volume =       "125",
    number =        "795",
    year =         "2003"
}

@article{Kaminski,
    author = "Kaminski, A.K., Caulfield, C.P., Taylor J.R.",
    title = "Transient growth in strongly stratified
    shear layers",
    journal =      "J. Fluid Mech.",
    volume =       "758",
    pages =        "R4",
    year =         "2014"
}

@article{Coelho,
    author = "Coelho, P.M. \& Pinho, F.T.",
    title = "A generalized Brinkman number for non-Newtonian duct flows",
    journal =      "J. Non-Newton. Fluid",
    volume =       "156",
    pages =        "202-206",
    year =         "2009"
}

@article{Tso_a,
    author = "Tso, C.P. \& Mahulikar, T.P.",
    title = "The use of the Brinkman number for single phase forced convective heat transfer in microchannels",
    journal =      "Int. J. Heat Mass Transf.",
    volume =       "42",
    pages =        "1813-1833",
    year =         "1999"
}

@article{Tso_b,
    author = "Tso, C.P. \& Mahulikar, T.P.",
    title = "The role of the Brinkman number in analysing flow transitions in microchannels",
    journal =      "Int. J. Heat Mass Transf.",
    volume =       "42",
    pages =        "1813-1833",
    year =         "1999"
}

@article{Orszag,
    author = "Orszag, S.",
    title = "Accurate solution of the Orr–Sommerfeld equation",
    journal =      "J. Fluid Mech.",
    volume =       "50",
    pages =        "689-703",
    year =         "1971"
}

@article{Farrell,
    author = "Farrell, B.F. \& Ioannou, P.J.",
    title = "Transient Development of Perturbations in Stratified Shear Flow",
    journal =      "J. Atmos. Sci.",
    volume =       "50",
    number =       "14",    
    pages =        "2201-2214",
    year =         "1993"
}

@article{Prigogine_2,
    author = "Glansdorff, I. \& Prigogine, P.",
    title = "On a general evolution criterion in macroscopic physics",
    journal =      "Physica",
    volume =       "30",
    pages =        "351-374",
    year =         "1964"
}

@article{Rebhan,
    author = "Rebhan, E.",
    title = "Maximum entropy production far from equilibrium: The example of strong shock waves",
    journal =      "Phys. Rev. A",
    volume =       "42",
    number =       "781",
    year =         "1990"
}

@article{Juretic,
    author = "Juretić, D. \& Županović, P.",
    title = "Photosynthetic models with maximum entropy production in irreversible charge transfer steps",
    journal =      "Comput. Biol. Chem.",
    volume =       "27",
    number =       "6",
    pages =        "541-553",
    year =         "2003"
}

@article{Paltridge,
    author = "Paltridge, G.W.",
    title = "Climate and thermodynamic systems of maximum dissipation",
    journal =      "Nature",
    volume =       "279",
    pages =        "630-631",
    year =         "1979"
}

@article{Ozawa,
    author = "Ozawa, H. \& Ohmura, N.",
    title = "The second law of thermodynamics and the global climate system: a review of the maximum entropy production principle",
    journal =      "Rev. Geophys.",
    volume =       "41",
    number =       "4",
    year =         "2003"
}

@article{LeDizes,
    author = "Le Dizès, S.",
    title = "Modal growth and non-modal growth in a stretched shear layer",
    journal =      "Eur. J. Mech. B Fluids",
    volume =       "22",
    pages =       "411-430",
    year =         "2003"
}

@article{Alizard,
    author = "Alizard, F., Robinet, J.C.",
    title = "Transient growth in a right-angled streamwise corner",
    journal =      "Eur. J. Mech. B Fluids",
    volume =       "37",
    pages =       "99-111",
    year =         "2013"
}

@article{Ayala,
    author = "Ayala, D., Protas, B.",
    title = "On maximum enstrophy growth in a hydrodynamic system",
    journal =      "Physica D",
    volume =       "37",
    pages =       "1553-1563",
    year =         "2011"
}

@article{DiVita,
    author = "Di Vita, A.",
    title = "Maximum or minimum entropy production? How to select a necessary criterion of stability for a dissipative fluid or plasma",
    journal =      "Phys. Rev. E",
    volume =       "81",
    number =       "041137",
    year =         "2010"
}

@article{Brandt,
    author = "Brandt, L.",
    title = "The lift-up effect: The linear mechanism behind transition and turbulence in shear flows",
    journal =      "Eur. J. Mech. B Fluids",
    volume =       "47",
    pages =       "80-96",
    year =         "2014"
}

@article{Nourgaliev,
    author = "Nourgaliev, R. \& Dinh, T. ",
    title = "The investigation of turbulence characteristics in an internally-heated unstably-stratified fluid layer",
    journal =      "Nucl. Engng. Design",
    volume =       "178",
    pages =       "235-258",
    year =         "1997"
}

@article{Kikuchi,
    author = "Kikuchi, Y., Shioyama, T. ",
    title = "Turbulent heat transport in a horizontal fluid layer
    heated internally and from below",
    journal =      "Int. J. Heat Mass Transf.",
    volume =       "29",
    pages =       "451-461",
    year =         "1986"
}

@article{Tritton,
    author = "Tritton, D. ",
    title = "Internally heated convection in the atmosphere of Venus and in the laboratory",
    journal =      "Nature",
    volume =       "257",
    pages =       "110-112",
    year =         "1975"
}

@article{Tritton_b,
    author = "Tritton, D. \& Zarraga, M. ",
    title = "Convection in horizontal layers with internal heat generation: experiments",
    journal =      "J. Fluid Mech.",
    volume =       "30",
    pages =       "21-32",
    year =         "1967"
}

@article{Orr,
    author = "Orr, W.M.",
    title = "The stability or instability of the steady motions of a perfect liquid and of a viscous liquid.",
    journal =      "Proc. R. Irish Acad. A",
    volume =       "27",
    pages =       "9-68",
    year =         "1907"
}

@article{Ellingsen,
    author = "Ellingsen, T. \& Palm, E.",
    title = "Stability of linear flow.",
    journal =      "Phys. Fluids",
    volume =       "18",
    pages =       "487",
    year =         "1975"
}

@article{Reddy,
    author = "Reddy, S.C. \& Henningson, D.S.",
    title = "Energy growth in viscous channel flows.",
    journal =      "J. Fluid Mech.",
    volume =       "252",
    pages =       "209-238",
    year =         "1993"
}

@article{Gustavsson,
    author = "Gustavsson, L.H.",
    title = "Energy growth of three-dimensional disturbances in plane Poiseuille flow.",
    journal =      "J. Fluid Mech.",
    volume =       "224",
    pages =       "241-260",
    year =         "1991"
}

@Book{Pazy,
  author = 	 "Pazy, A. ",
  title = 	 "Semigroups of linear operators andapplication to partial differential equations.",
  year = 	 "1983",
  publisher = "Springer"
}

%% End of file `jfm2esam.bib'.

